Solar abundance problem

The chemical composition of the Sun is among the most important quantities in astrophysics. Solar abundances are needed for modelling stellar atmospheres, stellar structure and evolution, population synthesis, and galaxies as a whole. The solar abundance problem refers to the conflict of observed data from helioseismology and the predictions made by stellar interior models for the Sun, if these models use the newest solar chemical composition obtained with 3D and NLTE models of radiative transfer. Here we take a close look at the problem from observational and theoretical perspective. We also provide a list of possible solutions, which have yet to be tested.

==> table.tex <==
\begin{deluxetable}{lcccc}
\tablewidth{0pt}
\tablecaption{Adopted solar chemical compositions. \label{tab:compo}} 
\tablehead{\colhead{} & \multicolumn{4}{c}{$\log{\epsilon}$} \\ 
\cline{2-5}
\\
\colhead{Element} & \colhead{GS98}  & \colhead{AGS05$^a$} & \colhead{AGSS09$^a$}
& \colhead{AGSS09ph$^b$}}\startdata
C & 8.52 & 8.39 & 8.43 & 8.43 \\
N & 7.92 & 7.78 & 7.83 & 7.83 \\
O & 8.83 & 8.66 & 8.69 & 8.69 \\
Ne & 8.08 & 7.84 & 7.93 & 7.93 \\
Na & 6.32 & 6.27 & 6.27 & 6.24 \\
Mg & 7.58 & 7.53 & 7.53 & 7.60 \\
Al & 6.49 & 6.43 & 6.43 & 6.45 \\   
Si & 7.56 & 7.51 & 7.51 & 7.51 \\
S & 7.20 & 7.16 & 7.15 & 7.12 \\ 
Ar & 6.40 & 6.18 & 6.40 & 6.40 \\ 
Ca & 6.35 & 6.29 & 6.29 & 6.34 \\ 
Cr & 5.69 & 5.63 & 5.64 & 5.64 \\
Mn & 5.53 & 5.47 & 5.48 & 5.43 \\
Fe & 7.50 & 7.45 & 7.45 & 7.50 \\
Ni & 6.25 & 6.19 & 6.20 & 6.22 \\
\enddata
\tablecomments{Abudances given  as $\log{\epsilon_i}\equiv\log{N_i/N_H}+12$.\\
  $^a$ The adopted abundances are the recommended solar photospheric abundances
  for  the volatile  elements  (C, N,  O, Ne  and  Ar) and  the CI  chondritic
  meteoritic values for the 
  remaining elements. 
  $^b$  The   adopted  abundances  are  the   recommended  solar  photospheric
  abundances throughout. } 
